Conservative Safety Monitors of Stochastic Dynamical Systems

Generating accurate runtime safety estimates for autonomous systems is vital to ensuring their continued proliferation. However, exhaustive reasoning about future behaviors is generally too complex to do at runtime. To provide scalable and formal safety estimates, we propose a method for leveraging design-time model checking results at runtime. Specifically, we model the system as a probabilistic automaton (PA) and compute bounded-time reachability probabilities over the states of the PA at design time. At runtime, we combine distributions of state estimates with the model checking results to produce a bounded time safety estimate. We argue that our approach produces well-calibrated safety probabilities, assuming the estimated state distributions are well-calibrated. We evaluate our approach on simulated water tanks.

==> commands.tex <==


\newtheorem{counterexample}{Counterexample}
\newtheorem*{remark}{Remark}

\DeclareMathOperator{\sign}{sgn}

% time step in our model, 1/freq
\newcommand{\timestep}{\ensuremath{\tau}\xspace}


\newcommand{\carlen}{\ensuremath{L}\xspace}

% MoS assumption
\newcommand{\mosa}{\ensuremath{\succeq_{MoS}^{PMC}}\xspace}
\newcommand{\mosaSMC}{\ensuremath{\succeq_{MoS}^{LSS}}\xspace}
\newcommand{\mosdist}{\ensuremath{\succeq_{d}}\xspace}
\newcommand{\mosspeed}{\ensuremath{\succeq_{v}}\xspace}
\newcommand{\moswl}{\ensuremath{\succeq_{\wl}}\xspace}
\newcommand{\mose}{\ensuremath{\succeq_{MoSE}}\xspace}

% bundle operation on the perception model
\newcommand{\bundleop}{\ensuremath{\operatorname{bndl}}\xspace} 

% generic aggregate symbol
\newcommand{\agg}{\ensuremath{G}\xspace} 

%%%% MODEL PARTS AND OUTCOMES %%% 

% path 
\newcommand{\ourpath}{\ensuremath{\pi}\xspace} 

% a set of paths
\newcommand{\pset}{\ensuremath{\Pi}\xspace} 

% outcome function
\newcommand{\outfn}{\ensuremath{\mathcal{o}}\xspace} 

% outcome trace
\newcommand{\outtr}{\ensuremath{o}\xspace} 

% set of outcome traces NOT NEEDED
%\newcommand{\outtrset}{\ensuremath{O}\xspace} 

% outcome labels
\newcommand{\outlabs}{\ensuremath{\mathcal{O}}\xspace}

% path relation based on outcomes
\newcommand{\pathrel}{\ensuremath{R}\xspace}

% outcome-based union
\newcommand{\union}{~\ensuremath{{\large \cup}\kern-0.5em\raisebox{0.75ex}{\tiny o}}~\xspace}

% outcome-based intersection
\newcommand{\intersec}{\xspace\ensuremath{{\large \cap}\kern-0.5em\raisebox{0.5ex}{\tiny o}}~\xspace}

% outcome-based set complement
\newcommand{\compl}{\xspace\ensuremath{{\large \setminus}\kern-0.2em\raisebox{0.5ex}{\tiny o}}~}

%{\large \setminus}\kern-0.2em\raisebox{0.5ex}{\tiny o}



%%%% SHIFTING %%%% 
% old state 
\newcommand{\oldstate}{\ensuremath{\bar{s}_b}\xspace}

% new state 
\newcommand{\newstate}{\ensuremath{\bar{s}_a}\xspace}

% old path set
\newcommand{\oldpset}{\ensuremath{\dot{\pset}_b}\xspace}

% new path set 
\newcommand{\newpset}{\ensuremath{\dot{\pset}_a}\xspace}


%%%% OLD SHIFTS %%%% 
% distance shift of a trace
\newcommand{\dshift}{\ensuremath{\operatorname{dshift}}\xspace} 
% speed shift of a trace
\newcommand{\sshift}{\ensuremath{\operatorname{sshift}}\xspace}


%%%% SUMMANDS %%%%

\newcommand{\sone}{\ensuremath{\mathsf{S1}}\xspace} 
\newcommand{\stwo}{\ensuremath{\mathsf{S2}}\xspace} 
\newcommand{\sthree}{\ensuremath{\mathsf{S3}}\xspace} 

%%%% AEBS %%%%

% PA Actions
\newcommand{\yesdet}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\nodet}{\ensuremath{\mathscr{M}}\xspace}
\newcommand{\emitdist}{\ensuremath{d}\xspace}
\newcommand{\intdet}{\ensuremath{\mathcal{I}}\xspace}

% low-level outcomes
\newcommand{\yeslldet}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\nolldet}{\ensuremath{\mathcal{N}}\xspace}

% safety property
\newcommand{\oursafeprop}{\ensuremath{\psi_{nocol}}\xspace}
% safety probability 
\newcommand{\oursafeprob}{\ensuremath{Pr_{nocol}}\xspace}

% unsafety property
\newcommand{\ourunsafeprop}{\ensuremath{\psi_{unsafe}}\xspace}
% unsafety probability 
\newcommand{\ourunsafeprob}{\ensuremath{Pr_{unsafe}}\xspace}



% crash probability 
\newcommand{\ourcrashprob}{\ensuremath{Pr_{col}}\xspace}

% detection probability 
\newcommand{\detprob}{\ensuremath{Pr_{det}}\xspace}


%%%% Water Tank %%%% 

% tank count 
\newcommand{\tankcount}{\ensuremath{J}\xspace}

% tank size 
\newcommand{\tanksize}{\ensuremath{TS}\xspace}

% true water level 
\newcommand{\wl}{\ensuremath{w}\xspace}

% perceived water level 
\newcommand{\wlp}{\ensuremath{\hat{w}}\xspace}

% inflow
\newcommand{\inflow}{\ensuremath{in}\xspace}

% outflow
\newcommand{\outflow}{\ensuremath{out}\xspace}

% upper threshold
\newcommand{\uct}{\ensuremath{UT}\xspace}

% lower threshold
\newcommand{\lct}{\ensuremath{LT}\xspace}

% error 
\newcommand{\err}{\ensuremath{e}\xspace}

% error window
\newcommand{\errwin}{\ensuremath{EW}\xspace}

% FULL value
\newcommand{\fulltank}{\ensuremath{FU}\xspace}

% EMPTY value
\newcommand{\emptytank}{\ensuremath{EM}\xspace}

% safety property 
\newcommand{\tanksafeprop}{\ensuremath{\psi_{\textit{flow}}}\xspace}

% time horizon for the safety property
\newcommand{\timebound}{\ensuremath{T}\xspace}


%%%% CONCRETE MODELS %%%%


% model 
\newcommand{\mdl}{\ensuremath{\mathsf{M}}\xspace}

\newcommand{\mdls}{\ensuremath{\mathbf{M}}\xspace}

% the original controller-plant model
\newcommand{\mcp}{\ensuremath{\mathsf{M}_{\text{cpl}}}\xspace}

% The perception/LEC model
\newcommand{\mper}{\ensuremath{\textsf{M}_{\text{per}}}\xspace}

% Any abstraction
\newcommand{\mabst}{\ensuremath{\mathsf{M}_{\text{abs}}}\xspace}

% The baseline abstraction
%\newcommand{\mba}{\ensuremath{\mathsf{M}_{\text{bas}}}\xspace}
\newcommand{\mba}{\ensuremath{\mathsf{M}_{\text{int}}}\xspace}

% The baseline abstraction with transition trimming
%\newcommand{\mbatt}{\ensuremath{\mathsf{M}_{\text{fldvnb}}}\xspace}
\newcommand{\mbatt}{\ensuremath{\mathsf{M}_{\text{tt}}}\xspace}

% The baseline abstraction with transition trimming
%\newcommand{\mbatt}{\ensuremath{\mathsf{M}_{\text{fldvnb}}}\xspace}
\newcommand{\mbattneg}{\ensuremath{\mathsf{M}_{\text{ttneg}}}\xspace}

% Matthew's lattice
%\newcommand{\mmc}{\ensuremath{\mathsf{M}_{\text{fldv}}}\xspace}
\newcommand{\mmc}{\ensuremath{\mathsf{M}_{\text{bun}}}\xspace}

% Ramneet's distance interval abstraction
%\newcommand{\mrk}{\ensuremath{\mathsf{M}_{\text{fedo}}}\xspace}
\newcommand{\mrk}{\ensuremath{\mathsf{M}_{\text{dr}}}\xspace}

% Exact model
%\newcommand{\mex}{\ensuremath{\mathsf{M}_{\text{ext}}}\xspace}
\newcommand{\mex}{\ensuremath{\mathsf{M}_{\text{exc}}}\xspace}

% Discrete model
%\newcommand{\mdisc}{\ensuremath{\mathsf{M}_{\text{fr}}}\xspace}
\newcommand{\mdisc}{\ensuremath{\mathsf{M}_{\text{sbtt}}}\xspace}

% insert tab
\newcommand\tab[1][1cm]{\hspace*{#1}}

% extra line in table cell
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
  

